A Study of the Scrum Master's Role

Scrum is an increasingly common approach to software development adopted by organizations around the world. However, as organizations transition from traditional plan-driven development to agile development with Scrum, the question arises as to which Scrum role (Product Owner, Scrum Master, or Scrum Team Member) corresponds to a Project Manager, or conversely which Scrum role should the Project Managers adopt? In an attempt to answer this question, we adopted a mixed-method research approach comprising a systematic literature review and embedded case study of a commercial software development team. Our research has identified activities that comprise the Scrum Master role, and which additional roles are actually performed by Scrum Masters in practice. We found nine activities that are performed by Scrum Masters. In addition, we found that Scrum Masters also perform other roles, most importantly as Project Managers. This latter situation results in tension and conflict of interest that could have a negative impact on the performance of the team as a whole. These results point to the need to re-assess the role of Project Managers in organizations that adopt Scrum as a development approach. We hypothesize that it might be better for Project Managers to become Product Owners, as aspects of this latter role are more consistent with the traditional responsibilities of a Project Manager.

==> data-extraction-form-table.tex <==

\centering
\begin{tabular}{p{5cm}p{7cm}}
\toprule
 \textbf{Research Methodology} &   \\
\midrule

Type of study & empirical, theoretical, unclear \\
Research method & qualitative, quantitative, mixed, descriptive  \\
Research sub-method & single case study, multiple case study, not applicable  \\
Means of data collection & survey, questionnaire, interview, literature  \\
Means of analysis & comparison, descriptive, measurement, classification  \\

\midrule
 \textbf{Empirical Project Features} &   \\
\midrule

Company size & multinational, SME, very small company \\
Application domain & Health, automotive, telecoms, education (etc) \\
Project distribution & co-located, distributed \\
Project duration &in year (1,2,...n) \\
Team Size & (\#) \\
Participants & industry, students, unclear \\
Scrum role & Scrum Master \\
Scrum activities & Particularly Scrum Master activities \\ 
\bottomrule
\end{tabular}


